Data-driven load disturbance rejection

Data-driven direct methods are still growing in popularity almost three decades after they were introduced. These methods use data collected from the process to identify optimal controller's parameters with little knowledge about the process itself. However, most of those works focus on the problem of reference tracking, whereas many of the problems faced in real-life are of disturbance rejection or attenuation. Also, the vastly majority of those works identify the parameters of linearly parametrized controllers, which amounts to fixing the poles of the controller's transfer function. Although the identification of the controller's poles is not prohibitive, as hinted by some of the papers, there is little effort on presenting a data-driven solution capable of doing so. With all that in mind, this work proposes a data-driven approach which is able to identify the zeros and the poles of a linear controller aiming at disturbance rejection. Two different one-step ahead predictors are proposed, one that is linear on the parameters and another that is non-linear. Also, two different techniques are employed to estimate the controller parameters, the first one minimizes the quadratic norm of the prediction error while the second one minimizes the correlation between the prediction error and an external signal. Simulations show the effectiveness of the proposed methods to estimate the optimal controller parameters of restricted order controllers aiming at disturbance rejection.

==> images/GNUmakefile <==
################################################################################
#  Makefile to generate the images for publishing
#  These programs must be installed:
#  - gnumake  (tested with version 4.2.1)
#  - pdflatex (tested with version 3.14159265-2.6-1.40.20 TeX Live 2019/Debian)
#  - inkscape (tested with versions 0.92 and 1.0)
#  - gnuplot  (tested with version 5.2 patchlevel 8)
#
#  Additionally, tested with
#       GNU bash version 5.0.17(1)-release in a Kubuntu 20.04
#       xmllint using libxml version 20910
#
#  This file version: 2020-10-04
#  Author: Roger W. P. da Silva (williandmn@gmail.com)
################################################################################

################################################################################
#                             V A R I A B L E S                                #
################################################################################
## Programs
# use bash with extended file pattern expansion enabled
 SHELL    := /bin/bash -O extglob

# LaTeX processor and command line parameters
TEX      := pdflatex
TEXFLAGS := -interaction=batchmode -halt-on-error

# SVG to PDF+LaTeX converter and command line parameters
INK      := inkscape
INKV    := $(INK) --version 2>&1 | grep '^Inkscape [0-9.]\+' | sed 's/^Inkscape \([0-9]\).*/\1/'
# since version 1.0 inkscape has changed the CLI options
MAJORV   := $(shell $(INKV))
ifeq "$(MAJORV)" "1"
    INKPDF := --export-filename
else
    INKPDF := --export-pdf
endif
INKFLAGS := --export-area-page --export-latex $(INKPDF)

# data to PDF+LaTeX plotting software and command line parameters
GP       := gnuplot
GPFLAGS  := -c

# grayscale
ROOT        := root
GS          := gs
GSFLAGS     := -sDEVICE=pdfwrite -dCompatibilityLevel=1.5 -dProcessDSCComments=false -dNOPAUSE -dQUIET -dBATCH
GSGRAYSCALE := -sProcessColorModel=DeviceGray -sColorConversionStrategy=Gray -dOverrideICC

## Directories and incude files
# Directories
SVGDIR  := svg
PDFDIR  := pdf
PLOTDIR := plots
DATADIR := $(PLOTDIR)/data
TEXDIR  := latex
# include files
PLOTH   := header.gp
TEXINC	:= template.tex

################################################################################
#                        I M P L I C I T   R U L E S                           #
################################################################################
## Disable these implicit rules for performance and debug purposes
# remove implicit suffixes
.SUFFIXES:

# remove additional implicit rules
%: %,v

%: RCS/%,v

%: RCS/%

%: s.%

%: SCCS/s.%

################################################################################
#                               T A R G E T S                                  #
################################################################################
## phony targets
.PHONY: all clean clean-latex clean-all debug

## real targets option A.1 (single plots)
# uncomment this if each *.plt file must generate only one *.pdf file
# PLOTS    := $(patsubst $(PLOTDIR)/%.plt,$(PDFDIR)/%.pdf,$(wildcard $(PLOTDIR)/*.plt))

## real targets option A.2 (multiple plots)
# uncomment this if a single *.plt file can generate multiple *.pdf files
# PLOTS    := $(patsubst $(DATADIR)/%.dat,$(PDFDIR)/%.pdf,$(wildcard $(DATADIR)/dcbt*-y.dat))\
#             $(patsubst $(DATADIR)/%.dat,$(PDFDIR)/%.pdf,$(wildcard $(DATADIR)/vdft*-y.dat))\
#             $(patsubst $(DATADIR)/%-y.dat,$(PDFDIR)/%.pdf,$(wildcard $(DATADIR)/exp*-y.dat))
PLOTS := $(PDFDIR)/boxplot-matching-vdft.pdf  $(PDFDIR)/boxplot-matching-dcbt.pdf \
         $(PDFDIR)/boxplot-mismatching-vdft.pdf  $(PDFDIR)/boxplot-mismatching-dcbt.pdf \
         $(PDFDIR)/boxplot-filter-vdft.pdf  $(PDFDIR)/boxplot-filter-dcbt.pdf \
         $(PDFDIR)/exp-matching-ol.pdf  $(PDFDIR)/exp-matching-cl.pdf \
         $(PDFDIR)/exp-mismatching-cl.pdf
#

## real targets option B (svg diagrams)
# uncomment this if there are *.svg files to be converted to *.pdf
DIAGRAMS := $(patsubst $(SVGDIR)/%.svg,$(PDFDIR)/%.pdf,$(wildcard $(SVGDIR)/*.svg))

## intermediate targets
# uncomment this to avoid deleting these LaTeX intermediate files
.PRECIOUS: $(patsubst $(PDFDIR)/%.pdf,$(TEXDIR)/%.tex,$(PLOTS) $(DIAGRAMS))

################################################################################
#                                R U L E S                                     #
################################################################################
## Main rule: generates all the PDF images.
#  Prerequisites:
#    - $(PLOTS)    = the PDF files with the plots initially from gnuplot scripts
#    - $(DIAGRAMS) = the PDF files with the diagrams initially from SVGs
all: $(PLOTS) $(DIAGRAMS)

## SVG to LaTeX: converts an SVG image into LaTeX and PDF using a LaTeX template.
#  Prerequisites:
#    - $(SVGDIR)/%.svg = an SVG file with line art and text
#    - $(TEXINC)       = a LaTeX file with the template model
#  Targets:
#    - $(TEXDIR)/%.tex         = a LaTeX file joining the two bellow:
#    - $(TEXDIR)/%-svg.pdf_tex = a LaTeX include file with the text
#    - $(TEXDIR)/%-svg.pdf     = a PDF file with the line art
$(TEXDIR)/%.tex $(TEXDIR)/%-svg.pdf_tex $(TEXDIR)/%-svg.pdf: $(SVGDIR)/%.svg $(TEXDIR)/$(TEXINC)
	$(INK) $(INKFLAGS) $(TEXDIR)/$(*F)-svg.pdf $< > /dev/null 2>&1 && \
	sed -e "s|<filename>|$(*F)-svg.pdf_tex|" $(TEXDIR)/$(TEXINC) > $(TEXDIR)/$(*F).tex
	(xmllint --xpath '//*[name()="dc:creator"]//*[name()="dc:title"]/text()' $< | xargs -I "{}" sed -i "s|<author>|{}|" $(TEXDIR)/$(*F).tex)
	@echo ""

## Gnuplot to LaTeX: converts a gnuplot script and a data file into LaTeX using
#    specific configurations (e.g. for option A.2).
#  Prerequisites:
#    - $(PLOTDIR)/%.plt = a GNUPLOT script with instructions to generate the plot
#    - $(PLOTH)         = a GNUPLOT include file with some common configuration
#    - $(DATADIR)/%.dat = a data file with data to be plotted
#  Targets:
#    - $(TEXDIR)/%.tex     = a LaTeX file with the text of the plot
#    - $(TEXDIR)/%-inc.pdf = a PDF file with the line art of the plot
# $(TEXDIR)/%.tex $(TEXDIR)/%-inc.pdf: $(PLOTDIR)/results.plt $(PLOTDIR)/$(PLOTH) $(DATADIR)/%.dat
# 	cd $(PLOTDIR) && \
# 	$(GP) $(GPFLAGS) results.plt $(*F)
# 	@echo ""
#
$(TEXDIR)/exp-%.tex $(TEXDIR)/exp-%-inc.pdf: $(PLOTDIR)/experiment.plt $(PLOTDIR)/$(PLOTH)
	cd $(PLOTDIR) && \
	$(GP) $(GPFLAGS) experiment.plt $(subst -, ,$(*F))
	@echo ""
#
$(TEXDIR)/boxplot-%.tex $(TEXDIR)/boxplot-%-inc.pdf: $(PLOTDIR)/boxplot.plt $(PLOTDIR)/$(PLOTH)
	cd $(PLOTDIR) && \
	$(GP) $(GPFLAGS) boxplot.plt $(subst -, ,$(*F))
	@echo ""
#
## Gnuplot to LaTeX: converts a gnuplot script and a data file into LaTeX using
#    a common configuration.
#  Prerequisites:
#    - $(PLOTDIR)/%.plt = a GNUPLOT script with instructions to generate the plot
#    - $(PLOTH)         = a GNUPLOT include file with some common configuration
#  Targets:
#    - $(TEXDIR)/%.tex     = a LaTeX file with the text of the plot
#    - $(TEXDIR)/%-inc.pdf = a PDF file with the line art of the plot
# $(TEXDIR)/%.tex $(TEXDIR)/%-inc.pdf: $(PLOTDIR)/%.plt $(PLOTDIR)/$(PLOTH)
# 	cd $(PLOTDIR) && \
# 	$(GP) $(GPFLAGS) $(*F).plt
# 	@echo ""

## Additional dependencies of the plots (e.g. data files, additional headers)
$(TEXDIR)/exp-cl.tex: $(DATADIR)/exp-cl-r.dat \
                      $(DATADIR)/exp-cl-u.dat \
                      $(DATADIR)/exp-cl-y.dat
#
$(TEXDIR)/exp-ol.tex: $(DATADIR)/exp-cl-u.dat \
                      $(DATADIR)/exp-cl-y.dat
#
$(TEXDIR)/boxplot-%-vdft.tex: $(DATADIR)/%/vdftlin-ol-j.dat \
                              $(DATADIR)/%/vdftlin-cl-j.dat \
                              $(DATADIR)/%/vdftnlin-ol-j.dat \
                              $(DATADIR)/%/vdftnlin-cl-j.dat
#
$(TEXDIR)/boxplot-%-vdft.tex: $(DATADIR)/%/dcbtlin-ol-j.dat \
                              $(DATADIR)/%/dcbtlin-cl-j.dat \
                              $(DATADIR)/%/dcbtnlin-ol-j.dat \
                              $(DATADIR)/%/dcbtnlin-cl-j.dat
#

## LaTeX to PDF: converts LaTeX and PDF files into self-contained PDF files.
#  Prerequisites:
#    - $(TEXDIR)/%.tex = a LaTeX file including the text and the line art
#  Targets:
#    - $(PDFDIR)/%.pdf = a final PDF file including the text and the line art
$(PDFDIR)/%.pdf: $(TEXDIR)/%.tex
	pushd $(TEXDIR) > /dev/null && \
	{ $(TEX) $(TEXFLAGS) $(<F) > /dev/null 2>&1 || { grep -e '^!' -A 3 $(*F).log && false; }; } && \
	rm $(*F).aux $(*F).log && \
	popd > /dev/null && \
	mv $(TEXDIR)/$(@F) $@
	@echo ""

## Soft cleaning: deletes the final PDF files generated.
clean:
	rm -f $(PLOTS) $(DIAGRAMS)

## LaTeX cleaning: deletes all files in the latex directory except the template.
clean-latex:
	rm -f $(TEXDIR)/!($(TEXINC))

## Full cleaning: removes the final PDFs and cleans the latex directory.
clean-all: clean-latex
	rm -f $(PDFDIR)/*.pdf

## Convert main PDF to grayscale
grayscale: all
	$(GS) $(GSFLAGS) $(GSGRAYSCALE) -sOutputFile=$(PDFDIR)/$(ROOT)_gray.pdf ../$(ROOT).pdf
	@echo ""

## Debug info: displays useful debugging information.
debug:
	@echo "Inkscape major ver.:   $(MAJORV)"
	@echo "Gnuplots folder:       $(PLOTDIR)/"
	@printf "Gnuplots headers:    $(addprefix \n                       ,$(PLOTH))"
	@echo ""
	@echo "LaTeX diagrams folder: $(TEXDIR)/"
	@printf "LaTeX template:      $(addprefix \n                       ,$(TEXINC))"
	@echo ""
	@echo "PDF images folder:     $(PDFDIR)/"
	@printf "PDF plots:           $(addprefix \n                       ,$(PLOTS))"
	@echo ""
	@printf "PDF diagrams:        $(addprefix \n                       ,$(DIAGRAMS))"
	@echo ""

